Optimizing Memory Performance of Xilinx FPGAs under Vitis

Plenty of research efforts have been devoted to FPGA-based acceleration, due to its low latency and high energy efficiency. However, using the original low-level hardware description languages like Verilog to program FPGAs requires generally good knowledge of hardware design details and hand-on experiences. Fortunately, the FPGA community intends to address this low programmability issues. For example, , with the intention that programming FPGAs is just as easy as programming GPUs. Even though Vitis is proven to increase programmability, we cannot directly obtain high performance without careful design regarding hardware pipeline and memory subsystem.In this paper, we focus on the memory subsystem, comprehensively and systematically benchmarking the effect of optimization methods on memory performance. Upon benchmarking, we quantitatively analyze the typical memory access patterns for a broad range of applications, including AI, HPC, and database. Further, we also provide the corresponding optimization direction for each memory access pattern so as to improve overall performance.

==> experiment.tex <==
\section{Empirical Evaluation}
\label{sec_experiment}
%In this section, we present the experimental setup, and then conduct intensive experiments to validate our observations. 

\subsection{Experimental Setup}
\label{subsec_experiment_stup}

{\bf System Architecture. }% Our target system is the second generation of the Intel Xeon+FPGA platform\cite{gupta2011harp}. 
We deploy BiS-KM on the second generation of the Intel Xeon+FPGA platform~\cite{gupta2011harp}, consisting of an Arria 10 FPGA and a Broadwell 14-core E5 processor on the same socket (Figure \ref{system_architecture}). 
The FPGA has cache-coherent access to the CPU's main memory (64GB) through 1 QPI and 2 PCIe links, reaching an aggregated maximum throughput of 17GB/s. We use the open-source framework Centaur~\cite{centaur} for software-hardware integration. Centaur manages the data communication between the FPGA and the CPU. BiS-KM is instantiated within Centaur as a User-Defined-Function.   

\begin{figure}[t]
	\centering
	\includegraphics[width=3.3in]{figure/system_archi.png}
	\vspace{-2.5ex}
	\caption{System architecture of the target platform}
	\vspace{-3ex}
	\label{system_architecture}
\end{figure} 

\noindent
{\bf Hardware Configuration. }%We adopt the hybrid memory layout with $PF$=16 as our BiS-KM memory layout.
% We configure the hybrid memory layout with $PF$=16. 
The hardware implementation in our experiment consists of $DISP=32$ pipelines, each of which accommodates a sample. Each pipeline is equipped with 8 Distance Processors to support a maximum of 8 clusters and each Distance Processor contains a BiS-DP unit to process 16 bits from 16 features ($DIFP=16$) per cycle. The maximum number of dimensions supported is 1024. The clocking frequency is 200MHz.    

\noindent
{\bf Workloads. }We run our experiments with four real-world data sets: OpenStreetMap~\cite{mapping}, Forest ~\cite{Forest}, Gas~\cite{gas} and Epileptic~\cite{epileptic}, as shown in Table~\ref{t_dataset}. The data sets cover a wide range of dimensions and are representative for clustering tasks. Because the original data set size of Gas, Epileptic and OpenStreetMap is small, we duplicate the original data (8 times, 8 times and 64 times respectively) in order to amortize the communication overhead between the CPU and the FPGA. Since the K-Means algorithm itself is sensitive to the initial centers, we use the same initial centers in all the experiments for each data set. %The details of each data set a shown in . 

\begin{table} [t]
\def\arraystretch{1.1}
	\centering
    \vspace{-0.5ex}
%	\begin{scriptsize}
	\caption{Evaluated data sets. }
	\label{t_dataset}
		\vspace{-1.5ex}
		\begin{tabular}{|c|c|c|c|}
			\hline
			\textbf{Data sets}& \textbf{Features} & \textbf{Samples} & \textbf{Clusters} \\
% 			\hline
% 			Household~\cite{household}&  7 &  2,049,280 & 8 \\
            \hline
			OpenStreetMap~\cite{mapping}&  28 &  674,944 & 6 \\
			\hline
			Forest~\cite{Forest}&  54 & 581,012 & 7 \\
			\hline
			Gas~\cite{gas}&  128 & 111,280 & 6\\		
			\hline
			Epileptic~\cite{epileptic}&  178 &  92,000 & 5\\
			\hline
		\end{tabular}
%	\end{scriptsize}
	\vspace{-3ex}
\end{table}

\noindent
{\bf Hardware Baseline. }To evaluate the effectiveness of our BiS-KM design, we choose the state-of-the-art flexible K-Means accelerator (Flex-KM)~\cite{flex-kmeans} as our baseline.\footnote{Actually, we re-implement Flex-KM on our Arria 10 FPGA according to the paper~\cite{flex-kmeans}. Our implementation can run at line rate (512 bits per cycle) with the same frequency of 200MHz.} %Running on the same platform and the same frequency, the baseline serves to highlight the impact on low precision and the design decisions made as part of BiS-KM. %due to the following reason. Both the BiS-KM design and our Flex-KM implementation run on the same platform, with the only difference that the Flex-KM runs in 32-bit precision while the BiS-KM runs in low precision. Therefore, we are able to accurately demonstrate the advantage of low-precision clustering enabled by BiS-KM, by avoiding unnecessary interfering factors such as FPGA type and memory bandwidth. %(2) The Flex-KM represents the state-of-the-art K-Means accelerator, on-the-par with a 10-core CPU. In our experiments, we deploy the Flex-KM on the same platform and clock it with the same frequency as the BiS-KM.  


\vspace{-1ex}
\subsection{Hardware Efficiency: Throughput}
\label{subsec_evaluation}
\vspace{-0.5ex}
In this subsection, we examine the hardware efficiency of the BiS-KM design in terms of throughput. The throughput is calculated by the data set size divided by the elapsed time required by an iteration. ``x-bit" means the BiS-KM design with an $x$-bit precision level, where $x$ varies from 1 to 32. %under different experiment conditions. %and elapsed time per iteration

% \noindent
% {\bf Throughput.} 
% Figure~\ref{Throughput} shows the throughput of the BiS-KM running with four data sets with different precision levels. There are several important observations. (1) We find out that throughput changes with different data sets. This is due to the fact that the samples are padded with zeros if the dimension is not a multiple of 16 because the BiS-DP consumes 16 features in parallel. The dimension of Household data set is padded from 7 to 16, meaning that about half of the bandwidth doesn't contain useful data and the throughput is roughly cut by half. Even though the Forest and the Epileptic data sets don't satisfy the dimension constraint, the influence on the throughput is minimal because these two data sets are of larger dimensions and the number of padded features only occupies a small portion of the whole. However, the dimension restriction is not a fundamental problem. It can be alleviated by using the BiS-DP consuming less features in parallel, with the trade-off of a higher resource consumption. (2) The throughput of Gas data set, which satisfies the dimension constraint, is reaching the theoretical maximum (512 bits at 200MHz gives 12.8GB/s), meaning that the design saturates the memory bandwidth. The reason for the throughput not getting exactly 12.8 GB/s is that the pipelines can not process sample bits during aggregation and center update stages. (3) The throughput is almost not affected by the precision level. This shows that with one storage layout and one hardware design, the BiS-KM can support any-precision computation at ease.   

\noindent\textbf{Effect of Dimensionality on Throughput. }We examine the effect of the number of dimensions on the achievable throughput. Under the BiS-KM memory layout, if the dimension of a data set is not a multiple of $DIFP$, we have to use zero padding to align it to $DIFP$, potentially wasting a certain amount of memory bandwidth due to the padding. Figure~\ref{Throughput} shows the throughput of BiS-KM on the four data sets for a varying number of dimensions. 

The throughput of BiS-KM varies only slightly with different dimensions. This is because the padding overhead is relatively small over the memory traffic between the FPGA and the host memory.  %different data sets. This is due to the fact that the samples are padded with zeros if the dimension is not a multiple of 16 because the BiS-DP consumes 16 features in parallel, i.e., the dimension of the OpenStreetMap data set padded from 28 to 32. However, the influence of the padded features on the throughput is minimal because the number of padded features only occupies a small portion of the whole. The dimension restriction problem can also be alleviated by using the BiS-DP consuming less features in parallel, with the trade-off of a higher resource consumption. 

The throughput of BiS-KM roughly reaches the theoretical memory bandwidth when the dimension of a data set is a multiple of $DIFP$=16. Take the data set Gas ($D$ = 128) as an example, BiS-KM can roughly saturate the FPGA's memory bandwidth, with its throughput close to the theoretical maximum bandwidth (512 bits at 200MHz is 12.8GB/s). However, there is still a small gap from the theoretical maximum bandwidth due to the fact that the computing pipelines are stalled in the global aggregation and division stages.
% that take a certain amount of cycles to finish. %which satisfies the dimension constraint, 



\begin{figure}[tb]
	\centering
	\includegraphics[width=3.2in]{figure/throughput.png}
	\vspace{-1.5ex}
	\caption{Throughput of different data sets running with various precision levels using BiS-KM}
	\vspace{-3ex}
	\label{Throughput}
\end{figure} 

\noindent
{\bf Effect of Precision Level. }Figure~\ref{speed_up_over_32} depicts the runtime speedups of different low-precision levels of BiS-KM over the 32-bit precision Flex-KM for four data sets. We make three observations.  

\begin{figure}[t]
 	\centering
 	\includegraphics[width=3.2in]{figure/speedup_over_32_new.png}
 	\vspace{-1.5ex}
 	\caption{Speedup of runtime per iteration of various low-precision over 32-bit precision computation}
 	\vspace{-3ex}
	\label{speed_up_over_32}
 \end{figure} 
\begin{figure}[t]
	\centering
	\vspace{-1.5ex}
	\subfloat[OpenStreetMap (28 features)]{\includegraphics[width=1.625in]{figure/map_mem_traffic.png} 
		\label{mem_household}} 
	\subfloat[Epileptic (178 features)]{\includegraphics[width=1.625in]{figure/epi_mem_traffic.png} 
		\label{mem_covertype}} 
		\vspace{-1.5ex}
		\caption{Memory traffic (bits) per sample as the precision varies}
		\label{mem_precision} 
	\vspace{-4ex}
\end{figure} 


First, BiS-KM achieves roughly linear speedup as the precision decreases, due to the linear reduction of memory traffic (Figure~\ref{mem_precision}). Thus, we conclude that the performance of BiS-KM is mainly bounded by the memory bandwidth between the CPU main memory and the FPGA. 

Second, the slightly sub-linear speedup observed at 4-bit precision level (Figure~\ref{speed_up_over_32}), is due to strided memory access, particularly when accessing the most significant four bits of every 32 bits. The DRAM's row buffer hit rate is about 4/32=12.5\%, affecting the achievable memory throughput.\footnote{The problem becomes worse at lower precision, e.g., a 2-bit precision, since the row buffer hit rate becomes even lower. Therefore, below 4-bits precision, the gains in hardware efficiency cannot amortize the losses in statistical efficiency. } 
%Figure \ref{speed_up_over_32} depicts the per-iteration runtime speedup of different low-precision levels of BiS-KM over the 32-bit precision Flex-KM for four data sets. We find out that we gain almost linearly speedup of runtime with the decrease of the precision level. The runtime benefit is brought by the reduction of the total data movement with lower bit level. 
% because the current design is bounded by the memory bandwidth between the CPU main memory and the FPGA. Nevertheless, the speedup is slightly sub-linear with 4-bit precision. As we reduce the precision, the memory access is no more sequential since some least significant bits are skipped, meaning that the row buffer locality of the DRAM is not fully exploited. This phenomenon gets more obvious with the lower precision because a larger jump of the memory access is required. 

Third, the actual throughput roughly stays the same with varying precision levels, as depicted in Figure~\ref{Throughput}, demonstrating that BiS-KM allows us to take full advantage of low precision. 

We conclude that BiS-KM is able to efficiently support any-precision clustering on the FPGA. %the BiS-KM hardware design efficiently supports any precision clustering. It means that

%Figure~\ref{Throughput} depicts the throughput of the BiS-KM on four data sets, when running in different precision levels. We observe that the throughput of each data set roughly stays the same with varying precision levels, demonstrating that the BiS-KM hardware design efficiently supports any precision clustering and then allow us to take full advantage of low precision. %This shows that by exploiting the bit-serial arithmetic, the BiS-KM hardware can support any-precision computation at ease.   




\vspace{-1.5ex}
\subsection{Statistical Efficiency: Loss vs. Iterations }
\label{subsection_connection}
\vspace{-0.5ex}

\begin{figure}[t]
	\centering
		%\vspace{-2ex}
	%\hfill
	\subfloat[OpenStreetMap (28 features)]{\includegraphics[width=1.625in]{figure/mappingloss_epoch.png} 
		\label{}} 
	\subfloat[Forest (54 features)]{\includegraphics[width=1.625in]{figure/covtypeloss_epoch.png} 
		\label{}} % \caption{}
		
	\hfill
	\subfloat[Gas (128 features)]{\includegraphics[width=1.625in]{figure/gasloss_epoch.png} 
		\label{}} 
	\subfloat[Epileptic (178 features)]{\includegraphics[width=1.625in]{figure/epiloss_epoch.png} 
		\label{loss_iteration_epi}} % \caption{}
	\vspace{-1.5ex}	
	\caption{Convergence comparison: training loss vs. iterations under various precision levels. In (d), the curve of 6-bit precision is out of the range of y-axis.} 
	\label{loss_iteration} 	
	%\vspace{-1ex}
\end{figure}  

We now examine the statistical efficiency of BiS-KM with different precision levels, in terms of loss (i.e., within-cluster sum of square error) vs. iterations (Figure~\ref{loss_iteration}). We use the 32-bit precision Flex-KM as our baseline. We make four observations. %We run the BiS-KM with four data sets under various precision levels and compare with the Flex-KM, as shown in Figure~\ref{loss_iteration}.

First, low precision levels do converge to the same loss as 32-bit precision. Figure~\ref{loss_iteration} illustrates that a 12-bit precision level is adequate to converge to the same loss as the 32-bit precision does, demonstrating the great advantage of leveraging low precision.

Second, a different data set can require a different minimum precision level to converge. Figure~\ref{loss_iteration} illustrates that the minimum precision level required by the OpenStreetMap, the Forest, the Gas and the Epileptic to converge to the same loss as 32-bit precision are 8 bits, 6 bits, 8 bits and 12 bits, respectively. This observation motivates our BiS-KM design allowing any-precision clustering with only one hardware implementation. %In order to fully take advantage of low-precision clustering, 

Third, a low precision level is able to successfully enter a smaller local minimum as the 32-bit precision does. Figure~\ref{loss_iteration} (b) illustrates that the BiS-KM design with a low-precision level is capable of following the transfer from a local minimum to a smaller local minimum for the data set Forest, indicating that the statistical efficiency can be preserved when using low precision data. 

Fourth, BiS-KM typically requires a similar number of iterations to converge to the same loss compared with the 32-bit precision Flex-KM. Figure~\ref{loss_iteration} shows that BiS-KM requires roughly the same number of iterations to converge as Flex-KM does for the data sets OpenStreetMap, Gas and Epiletptic. 

We conclude that the low-precision clustering enabled by BiS-KM can preserve the statistical efficiency. 

%Besides, all the data sets except the Forest requires similar iterations as the Flex-KM to converge. During the clustering process of the Forest, the cluster centers move from one local minimum to another better one. The BiS-KM is capable to keep track of the change of local minimum while it takes more iterations. Therefore, we conclude that the statistical efficiency can be well preserved with the BiS-KM.




\subsection{End-to-End Comparison: Loss vs. Time}

\begin{figure}[t]
	\centering
		%\vspace{-2ex}
	%\hfill
	\subfloat[OpenStreetMap (28 features)]{\includegraphics[width=1.625in]{figure/mappingloss_runtime.png} 
		\label{runtime_household}} 
	\subfloat[Forest (54 features)]{\includegraphics[width=1.625in]{figure/covtypeloss_runtime.png} 
		\label{runtime_covertype}} % \caption{}
		
	\hfill
	\subfloat[Gas (128 features)]{\includegraphics[width=1.625in]{figure/gasloss_runtime.png} 
		\label{runtime_gas}} 
	\subfloat[Epileptic (178 features)]{\includegraphics[width=1.625in]{figure/epiloss_runtime.png} 
		\label{runtime_epi}} % \caption{}
	\vspace{-1.5ex}	
	\caption{End-to-end comparison: training loss vs. runtime under various precision levels. In (d), the curve for 6-bit precision is out of the range of y-axis.} 
	\label{loss_runtime} 	
	%\vspace{-1ex}
\end{figure} 

In this subsection, we validate that BiS-KM with the low-precision dataset outperforms the 32-bit precision Flex-KM, in terms of end-to-end convergence rate. %performance loss vs. runtime). 
Figure ~\ref{loss_runtime} shows the convergence trends, loss vs. runtime, with various precision levels for four data sets. We observe that low precision leads to a significantly faster convergence rate. 
For the data sets OpenStreetMap, Forest and Gas, BiS-KM can achieve about 4X speedup to reach the same loss as the 32-bit precision Flex-KM does. However, BiS-KM can only achieve roughly 2.5X speedup for the data set Epileptic, which requires a 12-bit precision to converge to the same training loss as Flex-KM does.


	
	

\subsection{Comparison with CPU Implementations}

\noindent{\bf CPU Baselines. }We choose a highly optimized multi-core AVX2-enhanced CPU implementation as our software baseline~\cite{bohm2017multi}. 
The software baseline is originally implemented with AVX2 64-bit double-precision instructions, labelled as ``CPU:64-bit double''. 
Actually, we try to achieve more data parallelism using two smaller vector types: \emph{vector float} and \emph{vector short}.\footnote{ Multiplication-related AVX2 instruction does not support \emph{vector char} type. Even when the dataset is in 8-bit precision, we cannot achieve more parallelism, since we have to pad to a 16-bit boundary for further computation. } Accordingly, we produce two more CPU baselines: ``CPU:32-bit float'' and ``CPU:16-bit fixed point'', to improve the performance of K-Means on CPUs. %To fully exploit SIMD parallelism, we further improve the original baseline and introduce another two versions working with floating-point and 16-bit fixed-point SIMD instructions respectively.    
% The original data format of the software implementation is 64-bit double, meaning that each time 4 64-bit data are loaded to the 256-bit AVX2 register to perform  We further optimize the CPU implementation to support 32-bit floating-point and 16-bit fixed-point data format. 

% Figure ~\ref{cpu_comparison} shows the runtime-per-iteration comparison between the CPU baseline and the BiS-KM, for the Gas and the Epileptic respectively. We run three versions of the multi-core CPU implementation with increasing number of cores. The BiS-KM runs with the lowest precision level that leads to the same loss as 32-bit precision for the two data sets respectively.  
\noindent{\bf Comparison Methodology. }Since all the K-Means implementations on CPUs have roughly the same statistical efficiency as BiS-KM running at a reasonable precision level, the hardware efficiency comparison is the main metric showing the efficiency of BiS-KM. 

\noindent{\bf Comparison of Hardware Efficiency. }Figure ~\ref{cpu_comparison} illustrates the runtime-per-iteration comparison between the three software implementations and BiS-KM with the lowest precision level that leads to the same loss as 32-bit precision does, for the Gas and the Epileptic data set.
% \footnote{Due to page limit, we only put the results of two data sets}
The CPU implementation with a smaller vector datatype leads to higher performance, since a smaller vector datatype yields more data-level parallelism using SIMD and induces less memory traffic. BiS-KM is faster than ``CPU:64-bit double'' and ``CPU:32-bit float'', even though the 14-core CPU has 60GB/s memory bandwidth while our FPGA has only roughly 15GB/s. This is because BiS-KM takes advantage of low precision, e.g., using 6-bit precision. BiS-KM has roughly the same performance as ``CPU:16-bit fixed point'' with 6 (or 8) cores, since the K-Means algorithm is able to take full advantage of task-level (e.g., multi-core) and data-level (e.g., 32-way SIMD) parallelism on the CPU. Note, if we implement BiS-KM on a larger FPGA, e.g., VCU118, which has more FPGA resources and higher memory bandwidth, BiS-KM's performance would improve. Nevertheless, the fact that the FPGA can compete with 14 cores demonstrates the feasibility and advantages of the proposed approach even in its current configuration.  %and  achieves 32-way parallelism and .   

\begin{figure}[t]
	\centering
		%\vspace{-2ex}
	%\hfill
	\subfloat[Gas]{\includegraphics[width=1.625in]{figure/gas_sw_cmp.png} 
		\label{}}
	\subfloat[Epileptic]{\includegraphics[width=1.625in]{figure/epi_sw_cmp.png} 
		\label{}} 
		\vspace{-2ex}
		\caption{Runtime comparison between three CPU implementations with increasing number of cores and BiS-KM with the lowest precision level that is able to converge. }
		\label{cpu_comparison}
	\vspace{-3ex}
\end{figure} 

%As we can see, the software gains performance benefit by packing more data into one SIMD register. The BiS-KM outperforms 14-core software implementations running with double-precision and floating-point SIMD instructions for both data sets. The BiS-KM performance of the Gas and the Epileptic equals 6-core and 8-core software implementation running with 16-bit fixed-point SIMD instructions respectively.    

\subsection{Resource Consumption Breakdown}

Table ~\ref{tab:resources} shows the resource consumption breakdown of four modules in the BiS-KM hardware design. ALMs and BRAMs (i.e., ``M20Ks'' in the Table) are mostly used 
% by on-chip centers in 
the cluster assignment and accumulation modules, while the DSP utilization is low since it is mainly used to calculate the squared $L^2$ norm in the center pre-processing module. 
Table ~\ref{tab:resources} also shows the resource consumption of the major components, e.g., Accu and Agg. We observe that each component requires a very small amount of FPGA resources. For example, each \emph{Dist} consumes about 0.1\% ALMs, allowing us to instantiate a massive amount of \emph{Dists} to process multiple cluster centers concurrently on the FPGA. %the design to scale out to keep the line rate and to process multiple centers concurrently.
% The ALMs are mostly used for the cluster assignment. 
\begin{table}[h]
 	 	\caption{Resource consumption breakdown of the BiS-KM hardware design with $DIFP$=16 and $\#pipe$=32 }
 	 	\vspace{-3ex}
 	 	\begin{small}
 		\begin{center}
 			\def\arraystretch{1.1}
 			\begin{tabular}{l|c|c |c}
			\textbf{Resources} & \textbf{ALMs} & \textbf{M20Ks} & \textbf{DSPs}\\
			\hline
			Center Norm & 786 (0.18\%) & 0 (0\%) & 48 (3.16\%)\\
% 			BiS-DP  & 379 (0.09\%) & 0 (0\%) & 0 (0\%) \\
			Dist & 452 (0.11\%) & 0  (0\%) & 0 (0\%) \\
			Accu & 1,789 (0.42\%) & 29 (3.75\%) & 0 (0\%)\\
% 			1x Pipeline & 8212 (1.92\%) & 35 (1.29\%) & 55 (3.62\%)\\
			Agg & 219 (0.05\%) & 3 (0.70\%) & 1 (0.07\%)\\
			Div & 846 (0.20\%) & 1 (0.03\%) & 0 (0\%)\\
			\hline
			\hline
			\hline			
			Center pre-processing & 1,357 (0.32\%) & 26 (0.78\%) & 49 (3.22\%) \\
			Cluster assignment & 115,522 (27.10\%)& 208 (6.21\%) & 0 (0\%) \\
			Accumulation & 57,466 (13.45\%) & 931 (27.79\%) & 1 (0.07\%) \\
			Division & 1,674 (0.39\%) & 14 (0.42\%) & 0 (0\%) \\
			\hline
			BiS-KM & 176,019 (41.26\%) & 1,179 (35.19\%) & 50 (3.29\%) \\
			\vspace{-3ex}
% 			Total for P=8 & 86614 & 20.27\% & 432 & 15.92\% & 441 & 29.05\%\\
% 			Total for P=16 & 171550 & 40.17\% & 856 & 31.55\% & 881 & 58.04\%\\
% 			\hline
% 			Centaur & 87047& 20.38\% & 429 & 15.81\% & 0 & 0\%\\
			\end{tabular}
 		\end{center}
 		\end{small}
 		\label{tab:resources}
 	\end{table}
 	



 

==> overview.tex <==


%\vspace{-1ex}
% \section{System Overview}
% \vspace{-0.5ex}

% \begin{figure}[ht]
% 	\centering
% 	\includegraphics[width=3.3in]{figure/system_archi.png}
% 	\vspace{-1.5ex}
% 	\caption{System architecture of the target platform}
% 	\vspace{-3ex}
% 	\label{system_architecture}
% \end{figure} 

% Our target platform is the second generation of the Intel Xeon+FPGA ~\cite{gupta2011harp}. As shown in Figure~\ref{system_architecture}, it contains an Arria 10 FPGA and a Broadwell 14-core E5 processor on the same socket. The FPGA has cache-coherent access to the CPU shared main memory region(64GB) through 1 QPI and 2 PCIe links, reaching an aggregated maximum throughput of 17GB/s. We use the open-source framework Centaur~\cite{centaur} for software-hardware integration. The centaur provides a piece of hardware and a thin layer of the software that manage the data communication between the FPGA and the CPU. The BiS-KM is instantiated in the framework Centaur as a User-Defined-Function.   

==> related_work.tex <==
\section{Related Work}
To our knowledge, BiS-KM is the first novel solution that incorporates algorithm, software and hardware designs to enable any-precision K-Means. We contrast closely related work with BiS-KM on 1) FPGA-accelerated K-Means, 2) fast bulk bit-wise operations and 3) low-precision DNN and ML. 
% BiS-KM is built on previous work from multiple domains. 
% \noindent\textbf{Bulk bit-wise operations}

% \noindent\textbf{Novel Memory Layout. } Novel main memory layouts ~\cite{bit_weaving,byteslice} are proposed to facilitate fast bulk bit-wise operations for various applications, such as database scan and low-precision machine learning. 

\noindent\textbf{FPGA-Accelerated K-Means. }There is a wide range of research on accelerating the K-Means with the FPGA for various applications. However, most of the existing approaches focus on high-precision input data ~\cite{saegusa2006fpga, wang2007k, gokhale2003kmean, estlick2001, hussain2012kmeans, wang2016melia, flex-kmeans, km_hpca16, triangle_inequility_kmeans, opencl_kmeans, choi2014mapreducekmeans, bioinformatics_kmeans}. %Among them, Tang et.al. ~\cite{opencl_kmeans} reports up to 11\,GB/s of throughput, which is close to our throughput. However, BiS-KM is superior in terms of end-to-end runtime.
% because low-precision data requires less data movement.
% Besides, many of them only offload parts of the K-Means algorithm (i.e. cluster assignment step) onto the FPGA ~\cite{gokhale2003kmean}~\cite{estlick2001}, leading to a large communication overhead between the CPU and the FPGA. In contrast, the BiS-KM is a complete design that implement the entire algorithm on the FPGA. 
Among these, there is very few work that has considered the low-precision K-Means. Estlick et al.~\cite{estlick2001} run the K-Means algorithm on the CPU over the truncated datasets, whose $B$ least significant bits are truncated, where $B$ is 4, 6, or 8. In contrast, BiS-KM enables any-precision K-Means clustering using a single FPGA design. %, In prior efforts   %Estlick et al.~\cite{estlick2001} has experiments on running the K-Means with truncated input and shows that truncating eight least significant bits has a negligible impact on the final clustering accuracy. However, their experiment covers at lowest 24-bit precision and their hardware architecture is not designed for processing low-precision data. We give a more detailed analysis of the statistical efficiency of the low-precision K-Means and the BiS-KM supports any precision levels with bit-serial arithmetic.

\noindent\textbf{Fast Bulk Bit-wise Operations. }A broad range of applications, such as database scans~\cite{bit_weaving, byteslice, ambit, bitwise_agg, hebe_icde18, vectorize_scan} and low-precision machine learning and neural networks~\cite{ml_weaving, finn_bnn, bismo} use fast bulk bit-wise operations to improve their performance. 
%Fast bulk bit-wise operations have been used in various applications, such as database scans~\cite{bit_weaving, byteslice, ambit, bitwise_agg, vectorize_scan} and low-precision machine learning and neural networks~\cite{ml_weaving, finn_bnn, bismo}. 
%Closest to BiS-KM is the work by Wang et al.~\cite{ml_weaving} and Li et al.~\cite{bit_weaving} to propose custom fine-grained memory layouts to accelerate generalized linear model training and database scan, respectively. 
Closest to BiS-KM is the work by Wang et al.~\cite{ml_weaving} that proposes a customized MLWeaving memory layout to facilitate the hardware design of low-precision generalized linear model training. 
%In contrast, BiS-KM employs algorithm-software-hardware co-design to enable efficient any-precision clustering on FPGAs. 
%In these efforts, some propose novel main memory layouts~\cite{bit_weaving, byteslice, ml_weaving} to facilitate bulk bit-wise operations. In particular, the hybrid memory layouts of the BiS-KM is inspired by MLWeaving ~\cite{ml_weaving} and BitWeaving~\cite{bit_weaving}. 
%However, the memory layout of BiS-KM is different from both of them because it is tailored to satisfy the access pattern and the resource requirement of the K-Means algorithm. 

\noindent\textbf{Low-Precision DNN and ML. }Hardware acceleration of deep neural networks~\cite{fpga_cnn_li_jing, fpga_cnn_yun_liang, cnn_jason_cong, fpga_cnn_luo_guojie, fpga_cnn_tshinghua} and machine learning algorithms~\cite{dt,Kara2018ColumnMLCM,doppopdb2} has been a common topic for many years. Recently, researchers focus shifts to use low-precision hardware to further accelerate these workloads because the statistical efficiency of these algorithms can be well preserved in low precision. 
% Previous work ~\cite{Stripes, bit_fusion_isca18, neural_cache_isca18, proteus_ics16} exploits the bit-level flexibility on the input data so as to reduce the training time. Many of the work also utilize the bit-serial arithmetic to compute the dot-product in the training process. There are recent efforts accelerating other machine learning algorithms using quantized data~\cite{sgd-kaan-fccm, ml_weaving, zipml}. One close work with the BiS-KM is the MLWeaving~\cite{ml_weaving}. The MLWeaving accelerates the generalized linear models with the flexible bit-level memory layout and the bit-serial processing. The hybrid memory layout of the BiS-KM is inspired by the MLWeaving but it is tailored to the K-Means algorithm. 
Plenty of low-precision designs~\cite{sgd-kaan-fccm, zipml, finn_bnn, vibnn_asplos18} 
%shidiannao_isca15, tpu_isca17,pudianao_asplos15,dadiannao_micro14,
focus on using a fixed quantization of data and a fixed-bitwidth accelerator to accelerate DNN and ML workloads, while other research work ~\cite{Stripes, bit_fusion_isca18,  bismo} 
%neural_cache_isca18, proteus_ics16, tartan_arxiv17
focuses on exploiting the bit-level precision variability of hardware arithmetic for interference. In contrast, BiS-KM focuses on any-precision K-Means clustering. %Among them, MLWeaving ~\cite{ml_weaving} is the closest work to BiS-KM. The MLWeaving accelerates the generalized linear models with the flexible bit-level memory layout and the bit-serial arithmetic. Compared with MLWeaving, BiS-KM focuses on a different workload (i.e., clustering) and the whole design is tailored to K-Means clustering. 

% Most existing work either processes floating point or fixed point values. Estlick et al.~\cite{estlick2001} showed that using fixed point arithmetic instead of floating point for the distance calculation has a negligible impact on the final accuracy.

% Most existing work either processes floating or fixed point values. Estlick et al.~\cite{estlick2001} showed that using fixed point instead of floating point for the distance calculation has a negligible impact on the final accuracy. Many existing work offloads only parts of the algorithm such as the assignment~\cite{gokhale2003kmean,estlick2001}. 
% The benefit of offloading the entire algorithm due to reduced communication with the CPU, was shown by \cite{liu2005kacu}.
% In addition to implementing the entire algorithm in the FPGA, our design provides runtime parametrization in terms of number of clusters and dimensions.

% Many existing work focuses on offloading only parts of the algorithm such as the assignment~\cite{gokhale2003kmean,estlick2001}. The benefit of offloading the entire algorithm, and thereby reducing communication with the CPU,  was shown by \cite{liu2005kacu}. In this work we implemented the entire algorithm in the FPGA. In addition our design provides flexibility at runtime in terms of the number of clusters and dimensions.

% Several recent efforts use OpenCL~\cite{tang2016acceleration,wang2016melia} to accelerate K-means clustering: \cite{tang2016acceleration} reports up to 11\,GB/s of throughput which is similar to ours but neglecting the data transfer between host and device. Such designs provide limited flexibility in the number of clusters, while the number of dimensions is fixed. Further, they target an accelerator deployment, whereas the design presented in this work targets hybrid architectures.
% Hussain et al.~\cite{hussain2012kmeans} provides a K-means implementation that achieves flexibility through partial reconfiguration allowing to change the distance function or run multiple K-means kernel on different data sets in parallel. The authors of~\cite{choi2014mapreducekmeans} show a distributed K-means implementation achieving up to 100\,MB/s throughput in an FPGA-accelerated clusters.



